Energy Shift with Coupling (ESC): a new quench protection method

Quench protection of full-size high-field accelerator magnets poses significant challenges. Maintaining the hot-spot temperature and peak voltage-to-ground within acceptable limits requires a protection system that quickly transitions most of the coil turns to the normal state. Existing magnet protection technologies, such as quench protection heaters or the Coupling Loss Induced Quench system (CLIQ), have been successfully applied. However, they both present shortcomings since they require either thin insulation between the heaters and the magnet conductor or direct electrical connections to the magnet coil. A novel quench protection method, Energy Shift with Coupling (ESC), is presented which can achieve excellent quench protection performance without the above-mentioned drawbacks. ESC relies on normal-conducting auxiliary coils strongly magnetically coupled with the magnet coils to protect. Upon quench detection capacitive units connected across such coils introduce a high current change in the auxiliary coils causing a rapid shift of magnet stored energy from the magnet coils to the auxiliary coils. This has three beneficial effects: sudden reduction of ohmic loss in the normal zone of the magnet conductor, introduction of high transient losses in the magnet conductor, thus causing a quick transition to the normal state, and extraction of a part of the magnet stored energy to the auxiliary coils. The applicability of the ESC concept on an existing magnet design is analyzed with electromagnetic and thermal transient simulations performed with the STEAM-LEDET program. The advantages and disadvantages of ESC are discussed and compared to other conventional quench protection methods. Simulation results show that ESC can be applied to protect full-scale magnets with reasonable requirements in terms of size and location of the auxiliary coils and of capacitive unit parameters.

==> Sust_2024_ESC_sentToArxiv_20240909/figureElectricalCircuitEquivalent.tex <==
% Custom command to write labeled nodes
\newcommand{\labelednode}[3][above]{
	\node[circle,draw,fill=purple!50,minimum size=2mm] (#2) at (#3) {};
	\node[#1,black] at (#2.west) {#2}; % White text for visibility on purple background
}

\begin{figure}[tp]
	\centering
	\begin{circuitikz}[line width=0.5pt]
		\centering
		
		\ctikzset{resistor = european}
		
		%		GRID (used for debugging)
%				\draw[step=0.1cm,gray,very thin] (0,-2) grid (16,4);
		
		% Each letter is  a column. Each number is a r5w.
		%		\coordinate[circle,fill=black] (A1) at ( 0.0, 4); % for debugging
		\coordinate (G1) at ( 0.0, 0.0-1.2);
		\coordinate (A1) at ( 0.0, 0.5-1.2);
		\coordinate (A2) at ( 0.0, 1.5-1.0);
		\coordinate (A3) at ( 0.0, 2.0-1.0);
		\coordinate (A4) at ( 0.0, 3.0-1.0);
		\coordinate (A5) at ( 0.0, 3.5);
		\coordinate (B1) at ( 2.0, -1.2);
		\coordinate (B2) at ( 2.0, -0.2);
		\coordinate (B3) at ( 2.0, 1.0);
		\coordinate (B4) at ( 2.0, 2.0-0.5);
		\coordinate (B5) at ( 2.0, 3.0);
		\coordinate (B6) at ( 2.0, 3.5);
		\coordinate (C1) at ( 6.0, 0.0-1.2);
		\coordinate (C2) at ( 6.0, 0.5-1.2);
		\coordinate (C3) at ( 6.0, 1.5-1.2);
		\coordinate (C4) at ( 6.0, 2.0-1.2);
		\coordinate (C5) at ( 6.0, 3.0-1.2);
		\coordinate (C6) at ( 6.0, 3.5);
		\coordinate (D4) at ( 8.2, 1.8);
		\coordinate (D5) at ( 8.2, 2.0);
		\coordinate (D6) at ( 8.2, 3.0);
		\coordinate (D7) at ( 8.2, 3.5);
		\coordinate (E2) at ( 8.5, 1.8);
		\coordinate (E3) at (11.0, 1.8);
		\coordinate (E4) at (12.0, 1.8);
		\coordinate (E5) at (12.0, 1.9);
		\coordinate (E6) at (12.0, 3.4);
		\coordinate (E7) at (12.0, 3.5);
		\coordinate (F4) at (14.5, 1.8);
		\coordinate (F8) at (14.5, 2.2);
		\coordinate (F5) at (14.5, 2.7);
		\coordinate (F6) at (14.5, 3.0);
		\coordinate (F7) at (14.5, 3.5);
		\coordinate (L1) at (14.35, 2.35);
		\coordinate (L2) at (14.6, 2.95);
		\coordinate (L3) at (14.5, 3.0);
		\coordinate (T1) at (14.0, 3.5);
		\coordinate (T2) at (14.0, 3.8);
		\coordinate (T3) at (13.0, 3.8);
		\coordinate (T4) at (13.0, 3.5);
		\coordinate (T5) at (13.0, 3.2);
		\coordinate (T6) at (14.0, 3.2);
		\coordinate (T7) at (13.1, 2.8);
		\coordinate (G4) at (15.5, 2.7);
		\coordinate (G5) at (15.5, 2.5);
		\coordinate (H1) at (14.75, 3.4);
		\coordinate (PS1) at (-0.3, 0.3);
		\coordinate (R1) at ( 2.8, 3.5);
		\coordinate (R2) at ( 2.8, -1.2);
		\coordinate[below=3cm of D4]  (D4b);
		\coordinate[below=3cm of D5]  (D5b);
		\coordinate[below=3cm of D6]  (D6b);
		\coordinate[below=3cm of D7]  (D7b);
		\coordinate[below=3cm of E2]  (E2b);
		\coordinate[below=3cm of E3]  (E3b);
		\coordinate[below=3cm of E4]  (E4b);
		\coordinate[below=3cm of E5]  (E5b);
		\coordinate[below=3cm of E6]  (E6b);
		\coordinate[below=3cm of E7]  (E7b);
		\coordinate[below=3cm of F4]  (F4b);
		\coordinate[below=3cm of F5]  (F5b);
		\coordinate[below=3cm of F6]  (F6b);
		\coordinate[below=3cm of F7]  (F7b);
		\coordinate[below=3cm of F8]  (F8b);
		\coordinate[below=3cm of L1]  (L1b);
		\coordinate[below=3cm of L2]  (L2b);
		\coordinate[below=3cm of L3]  (L3b);
		\coordinate[below=3cm of T1]  (T1b);
		\coordinate[below=3cm of T2]  (T2b);
		\coordinate[below=3cm of T3]  (T3b);
		\coordinate[below=3cm of T4]  (T4b);
		\coordinate[below=3cm of T5]  (T5b);
		\coordinate[below=3cm of T6]  (T6b);
		\coordinate[below=3cm of T7]  (T7b);
		\coordinate[below=3cm of G4]  (G4b);
		\coordinate[below=3cm of G5]  (G5b);
		\coordinate[below=3cm of H1]  (H1b);
		\coordinate[below=3cm of PS1]  (PS1b);
		\coordinate (M1) at ( 6.3, 1.4);
		\coordinate (M2) at ( 6.3, 1.2);
		\coordinate (M3) at ( 7.9, 2.3);
		\coordinate (P1) at ( 5.8, 1.7);
		\coordinate (P2) at ( 8.35, 2.89);
		\coordinate (P3) at ( 8.35, -0.1);
		\coordinate (Z1) at ( 8.5, 0.6);
		\coordinate (Z2) at ( 8.5, 1.2);
		\coordinate (Z3) at ( 8.5, 1.9);
		\coordinate (Z4) at ( 8.5, 2.5);
		\coordinate (Z5) at (12.0, 2.5);
		\coordinate (Z6) at (12.0, 0.6);
		\coordinate (Z7) at (10.3, 2.7);
		
		
		% Magnet circuit
		\draw[color=black] (G1) to (A1)
		to [/tikz/circuitikz/bipoles/length=20pt, european voltage source, l=PS] (A2)
		to (A3)
		to[opening switch, o-o, l=SW, mirror] (A4);
%		\draw[color=black, very thick, o-o] (A3) to (A4); % this is ment to reproduce a closed switch
		\node[] at (PS1) {+};
		\draw[color=black] (A4) to (A5)
		to (B6)
		to [/tikz/circuitikz/bipoles/length=20pt, R, l=R$\st{circuit}$, i=$I\st{m}$] (C6);
		\draw[color=black] (G1) to (B1)
		to (B2)
		to [/tikz/circuitikz/bipoles/length=20pt, D, l=D$\st{crowbar}$] (B3)
		to (B4)
		to [/tikz/circuitikz/bipoles/length=20pt, R, l=R$\st{crowbar}$] (B5)
		to (B6);
		\draw[color=black] (B1) to (C1)
		to (C2)
		to [/tikz/circuitikz/bipoles/length=20pt, vR, invert, l=R$\st{m}$] (C3)
		to (C4)
		to [/tikz/circuitikz/bipoles/length=30pt, L, mirror, l=L$\st{m}$] (C5)
		to (C6);
		% Reverse PC Diode
		\draw[color=black] (R1)
		to [/tikz/circuitikz/bipoles/length=20pt, D, l=D$\st{rev}$] (R2);
		\draw[color=black] (G1) node[ground]{};
		
		% Auxiliary coil 1
		\draw[color=black] (D4)
		to (E2)
		to [/tikz/circuitikz/bipoles/length=20pt, vR, mirror, l=R$\st{1}$, i=$I\st{1}$] (E3)
		to (E4)
		to [/tikz/circuitikz/bipoles/length=20pt, D, l=D$\st{1}$, i=$I\st{D1}$] (E6)
		to (E7)
		to (D7)
		to (D6)
		to [/tikz/circuitikz/bipoles/length=30pt, L, mirror, l=L$\st{1}$] (D5)
		to (D4);
		% ESC unit 1
		\draw[color=black] (E4) to [/tikz/circuitikz/bipoles/length=15pt, R, l=R$\st{c1}$, i=$I\st{c1}$] (F4)
		to (F8)
		to [/tikz/circuitikz/bipoles/length=15pt, C] (F5)
		to [/tikz/circuitikz/bipoles/length=15pt, C] (F6)
		to (F7);
		% ESC capacitor bank
		\node[draw, rectangle, fit={(L1) (L2)}] {};
		\node at (L1) [right=2mm of L3] {C$\st{c1}$}; % label
		% ESC back-to-back thyristors		
		\draw[color=black]  (F7)
		to (T1)
		to (T2)
		to [/tikz/circuitikz/bipoles/length=0.5cm,thyristor] (T3)
		to (T4)
		to (E7);
		\draw[color=black] 
		(T4)
		to (T5)
		to [/tikz/circuitikz/bipoles/length=0.5cm, thyristor] (T6)
		to (T1);
		\node at (T7) [right=0mm of T7] {T$\st{c1}$}; % label
		
		
%		\draw[color=black] (E3) to (F4) to (F7) to (E7);
		\draw[color=black] (F5) to (G4) to (G5);
		\draw[color=black] (G5) node[ground]{};
%		\node at (F5) [rectangle,draw,fill=white] (v100) {ESC$\st{1}$};
		\node[] at (H1) {+};
		
		% Auxiliary coil 2
		\draw[color=black] (D4b)
		to (E2b)
		to [/tikz/circuitikz/bipoles/length=20pt, vR, mirror, l=R$\st{2}$, i=$I\st{2}$] (E3b)
		to (E4b)
		to [/tikz/circuitikz/bipoles/length=20pt, D, l=D$\st{2}$, i=$I\st{D2}$] (E6b)
		to (E7b)
		to (D7b)
		to (D6b)
		to [/tikz/circuitikz/bipoles/length=30pt, L, mirror, l=L$\st{2}$] (D5b)
		to (D4b);
		\draw[color=black] (E4b) to [/tikz/circuitikz/bipoles/length=15pt, R, l=R$\st{c2}$, i=$I\st{c2}$] (F4b)
		to (F8b)
		to [/tikz/circuitikz/bipoles/length=15pt, C] (F5b)
		to [/tikz/circuitikz/bipoles/length=15pt, C] (F6b)
		to (F7b);
		% ESC capacitor bank
		\node[draw, rectangle, fit={(L1b) (L2b)}] {};
		\node at (L1b) [right=2mm of L3b] {C$\st{c2}$}; % label
		\draw[color=black] (F5b) to (G4b) to (G5b);
		\draw[color=black] (G5b) node[ground]{};
%		\node at (F5b) [rectangle,draw,fill=white] (v100) {ESC$\st{2}$};
		\node[] at (H1b) {+};
		% ESC back-to-back thyristors		
		\draw[color=black]  (F7b)
		to (T1b)
		to (T2b)
		to [/tikz/circuitikz/bipoles/length=0.5cm,thyristor] (T3b)
		to (T4b)
		to (E7b);
		\draw[color=black] 
		(T4b)
		to (T5b)
		to [/tikz/circuitikz/bipoles/length=0.5cm, thyristor] (T6b)
		to (T1b);
		\node at (T7b) [right=0mm of T7b] {T$\st{c2}$}; % label

		% Mutual coupling
		\draw [<->,>=stealth] (M1)  to [bend left]  node[pos=0.5,fill=white] {M$\st{m,1}$} ++(1.6,+1.1);
		\draw [<->,>=stealth] (M2)  to [bend right] node[pos=0.5,fill=white] {M$\st{m,2}$} ++(1.6,-1.7);
		\draw [<->,>=stealth] (M3)  to [bend right] node[pos=0.5,fill=white] {M$\st{1,2}$} ++(0.0,-2.6);
		% Add circles indicating mutual coupling polarity
		\node[circle,draw=black,fill=black,minimum size=3pt,inner sep=0pt] at (P1) {};
		\node[circle,draw=black,fill=black,minimum size=3pt,inner sep=0pt] at (P2) {};
		\node[circle,draw=black,fill=black,minimum size=3pt,inner sep=0pt] at (P3) {};

%		% Add circles at nodes
		\node[circ] at (G1) {};
		\node[circ] at (B1) {};
		\node[circ] at (B6) {};
		\node[circ] at (R1) {};
		\node[circ] at (R2) {};
		\node[circ] at (E4) {};
		\node[circ] at (E7) {};
		\node[circ] at (E4b) {};
		\node[circ] at (E7b) {};
		
%		% Add blue patch for the cryogenic parts
%		\begin{scope}
%			\fill[blue!20, opacity=0.3] (4.7,-1.7) rectangle (11.0,4.2);
%		\end{scope}
%		\begin{scope}
%			\fill[magenta!20, opacity=0.3] (11.0,-1.7) rectangle (12.7,4.2);
%		\end{scope}
%		
		\draw[blue] (4.7,-1.7) rectangle (10.8,4.2);
		\draw[magenta] (11.0,-1.7) rectangle (12.7,4.2);


		% for debugging
%		\labelednode[above]{G1}{G1}
%		\labelednode[above]{A1}{A1}
%		\labelednode[above]{A2}{A2}
%		\labelednode[above]{A3}{A3}
%		\labelednode[above]{A4}{A4}
%		\labelednode[above]{A5}{A5}
%		\labelednode[above]{B1}{B1}
%		\labelednode[above]{B2}{B2}
%		\labelednode[above]{B3}{B3}
%		\labelednode[above]{B4}{B4}
%		\labelednode[above]{B5}{B5}
%		\labelednode[above]{B6}{B6}
%		\labelednode[above]{C1}{C1}
%		\labelednode[above]{C2}{C2}
%		\labelednode[above]{C3}{C3}
%		\labelednode[above]{C4}{C4}
%		\labelednode[above]{C5}{C5}
%		\labelednode[above]{D4}{D4}
%		\labelednode[above]{E2}{E2}
%		\labelednode[above]{E3}{E3}
%		\labelednode[above]{E4}{E4}
%		\labelednode[above]{E5}{E5}
%		\labelednode[above]{E6}{E6}
%		\labelednode[above]{E7}{E7}
%		\labelednode[above]{H1}{H1}
%		\labelednode[above]{H2}{H2}
%		\labelednode[above]{H3}{H3}
%		\labelednode[above]{H4}{H4}
%		\labelednode[above]{H5}{H5}
%		\labelednode[above]{H6}{H6}
%		

		
		% Add capacitor polarity
		
		
	\end{circuitikz}
%	\put(-480, 85){\color{black}{SW}}


	\caption{Simplified electrical scheme of the circuit including a magnet protected by two ESC coils.
		The magnet circuit includes a power supply (PS), a switch (SW) that opens when PS is switched off, a crowbar composed of a resistor R$\st{crowbar}$ and a diode D$\st{crowbar}$, a reverse diode D$\st{rev}$ to protect the PS, warm circuit resistance R$\st{circuit}$, and a magnet with its inductance L$\st{m}$ and resistance R$\st{m}$.
		Each ESC circuit includes: auxiliary coils with their inductances (L$_1$, L$_2$) and resistances (R$_1$, R$_2$); an ESC unit composed of a capacitor bank grounded in its mid-point (C$\st{c1}$, C$\st{c2}$), an internal resistance (R$\st{c1}$, R$\st{c2}$) and back-to-back triggering thyristors (T$\st{c1}$, T$\st{c2}$); and a diode (D$_1$, D$_2$).
		The coils $L\st{m}$, $L_1$, and $L_2$ are mutually coupled.
		The blue rectangle identifies the parts of the circuit at cryogenic temperature.
		The ESC diodes (magenta rectangle) can be located either in the room temperature or cryogenic part of the circuit.
		}
	\label{fig_circuit}
\end{figure}
%
